Cyclotomic Aperiodic Substitution Tilings

The class of Cyclotomic Aperiodic Substitution Tilings (CAST) is introduced. Its vertices are supported on the 2n-th cyclotomic field. It covers a wide range of known aperiodic substitution tilings of the plane with finite rotations. Substitution matrices and minimal inflation multipliers of CASTs are discussed as well as practical use cases to identify specimen with individual dihedral symmetry Dn or D2n, i.e. the tiling contains an infinite number of patches of any size with dihedral symmetry Dn or D2n only by iteration of substitution rules on a single tile.

==> hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump


